Dihadron correlations in PbPb collisions at 2.76 TeV with CMS

Measurements of charged dihadron DeltaEta-DeltaPhi correlations from the CMS collaboration are presented for PbPb collisions at a center-of-mass energy of 2.76 TeV per nucleon pair over a broad range of pseudorapidity and the full range of azimuthal angle. A significant correlated yield is observed for pairs of particles with small DeltaPhi but large longitudinal separation DeltaEta, commonly known as the "ridge". The ridge persists up to at least |DeltaEta| = 4 and the dependence of the ridge region shape and yield on collision centrality and transverse momentum has been measured. A Fourier analysis of the long-range two-particle correlation is presented and discussed in the context of higher order flow coefficients.

==> custom-definitions.tex <==
%
% custom definitions
%
\newcommand {\roots}    {\ensuremath{\sqrt{s}}}
\newcommand {\rootsNN}  {\ensuremath{\sqrt{s_{_{NN}}}}}
\newcommand {\dndy}     {\ensuremath{dN/dy}}
\newcommand {\dnchdy}   {\ensuremath{dN_{\mathrm{ch}}/dy}}
\newcommand {\dndeta}   {\ensuremath{dN/d\eta}}
\newcommand {\dnchdeta} {\ensuremath{dN_{\mathrm{ch}}/d\eta}}
\newcommand {\dndpt}    {\ensuremath{dN/d\pt}}
\newcommand {\dnchdpt}  {\ensuremath{dN_{\mathrm{ch}}/d\pt}}
\newcommand {\deta}     {\ensuremath{\Delta\eta}}
\newcommand {\dphi}     {\ensuremath{\Delta\phi}}
\newcommand {\pttrg}       {\ensuremath{p_T^{\mathrm{trig}}}}
\newcommand {\ptass}       {\ensuremath{p_T^{\mathrm{assoc}}}}
\newcommand {\AJ}       {\ensuremath{A_J}}
\newcommand {\npart}    {\ensuremath{N_{part}}}
\newcommand {\ncoll}    {\ensuremath{N_{coll}}}
%\newcommand {\ET}       {\ensuremath{E_T}}  %% already defined in ../../../utils/trunk/general/ptdr-definitions.tex

\newcommand {\pp}    {\mbox{pp}}
\newcommand {\ppbar} {\mbox{p\={p}}}
\newcommand {\pbarp} {\mbox{p\={p}}}
\newcommand {\PbPb}  {\mbox{PbPb }}


\newcommand{\m}{\ensuremath{\,\text{m}}\xspace}

\newcommand {\naive}    {na\"{\i}ve}
\providecommand{\GEANT} {{Geant}\xspace}
\providecommand{\PHOJET} {\textsc{phojet}\xspace}

% roman d for derivatives
\def\d{\mathrm{d}}

% pennames
\providecommand{\PKzS}{\ensuremath{\mathrm{K^0_S}}}
\providecommand{\Pp}{\ensuremath{\mathrm{p}}}
\providecommand{\Pap}{\ensuremath{\mathrm{\overline{p}}}}
\providecommand{\PgL}{\ensuremath{\Lambda}}
\providecommand{\PagL}{\ensuremath{\overline{\Lambda}}}
\providecommand{\PgS}{\ensuremath{\Sigma}}
\providecommand{\PgSm}{\ensuremath{\Sigma^-}}
\providecommand{\PgSp}{\ensuremath{\Sigma^+}}
\providecommand{\PagSm}{\ensuremath{\overline{\Sigma}^-}}
\providecommand{\PagSp}{\ensuremath{\overline{\Sigma}^+}}
\renewcommand{\GEANTfour} {{Geant4}\xspace}

